A Framework for the Automated Verification of Algebraic Effects and Handlers (extended version)

Algebraic effects and handlers are a powerful abstraction to build non-local control-flow mechanisms such as resumable exceptions, lightweight threads, co-routines, generators, and asynchronous I/O. All of such features have very evolved semantics, hence they pose very interesting challenges to deductive verification techniques. In fact, there are very few proposed techniques to deductively verify programs featuring these constructs, even fewer when it comes to automated proofs. In this paper, we present an extension to Cameleer, a deductive verification tool for OCaml code, that allows one to reason about algebraic effects and handlers. Our proposal embeds the behavior of effects and handlers using exceptions and employs defunctionalization to deal with continuations exposed by effect handlers.

==> mymacros.tex <==
\newcommand{\ity}[9]{#1\cdot#2\cdot#3\cdot#4\vdash #5:#6\cdot#7\cdot#8\cdot#9}

\newcommand{\whyml}{\textsf{WhyML}\xspace}
\newcommand{\kidml}{\textsf{KidML}\xspace}
\newcommand{\ocaml}{\textsf{OCaml}\xspace}
\newcommand{\dafny}{\textsf{Dafny}\xspace}
\newcommand{\mixins}{{Mixins}\xspace}
\newcommand{\coq}{\textsf{Coq}\xspace}
\newcommand{\clang}{{C}\xspace}
\newcommand{\cfml}{\textsf{CFML}\xspace}
\newcommand{\vocal}{\textsf{VOCaL}\xspace}
\newcommand{\osl}{\textsf{OSL}\xspace}
\newcommand{\why}{\textsf{Why3}\xspace}
\newcommand{\focalize}{\textsf{FoCaLiZe}\xspace}
\newcommand{\viper}{\textsf{Viper}\xspace}

\definecolor{thegray}{rgb}{0.9,0.9,0.9}
\definecolor{colorspec}{rgb}{0,0,0.797}
\definecolor{thered}{rgb}{0.797,0,0}
\definecolor{darkgreen}{rgb}{0.797,0,0}
\definecolor{theblue}{rgb}{0,0,0.797}
%\definecolor{thegray}{rgb}{0.949,0.949,0.949}
\definecolor{darkgray}{rgb}{0.8477,0.8477,0.8477}
\definecolor{ocaml-bg}{rgb}{0.9,0.9,0.9}
\definecolor{thegraygray}{rgb}{0.5,0.5,0.5}

% \DeclareCaptionFormat{listing}{\hfill#3}
% \captionsetup[lstlisting]{format=listing,singlelinecheck=false, margin=0pt,
%   font={sf,it,footnotesize},labelsep=space,labelfont=bf,belowskip=-1pt}

\newenvironment{judge}[2][c]
{\begin{minipage}[#1]{#2}
\hrule height2pt
\centerline{\vrule width2pt height 5pt\hfill \vrule width2pt height 5pt}
\begin{minipage}{\dimexpr\textwidth-4pt-1em}}
{\end{minipage}
\centerline{\vrule width2pt height 5pt\hfill \vrule width2pt height 5pt}
\hrule height2pt
\end{minipage}}

\newcommand{\todoi}[1]{\todo[inline]{#1}}

%%% syntax %%%
\newcommand{\taubar}{\overline{\tau}}
\newcommand{\btau}{\beta\tau}
\newcommand{\betaxbar}{\overline{\beta x}}
\newcommand{\betapxbar}{\overline{\beta' x}}
\newcommand{\btaubar}{\overline{\btau}}
\newcommand{\bitaubar}[1]{\overline{\beta_{#1}\tau}}
\newcommand{\bitauibar}[2]{\overline{\beta_{#1}\tau_{#2}}}
\newcommand{\bibar}[1]{\overline{\beta_{#1}}}
\newcommand{\bibarp}[1]{\overline{\beta_{#1}'}}
\newcommand{\bibarpp}[1]{\overline{\beta_{#1}''}}
\newcommand{\btaubarp}{\overline{\btau'}}
\newcommand{\bptaubar}{\overline{\beta'\tau}}
\newcommand{\bpptaubar}{\overline{\beta''\tau}}
\newcommand{\betabar}{\overline{\beta}}
\newcommand{\betabarp}{\overline{\beta'}}
\newcommand{\betabarpp}{\overline{\beta''}}
\newcommand{\betaibar}{\overline{\beta_i}}
\newcommand{\bitau}{\overline{\beta_i\tau_i}}
\newcommand{\bitaup}{\overline{\beta_i'\tau_i}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\pibari}[1]{\overline{\pi_{#1}}}
\newcommand{\xbart}[1]{\overline{x:#1}}
\newcommand{\xpibar}{\overline{x:\pi}}
\newcommand{\pebar}{\overline{\bar{p}\Rightarrow e}}
\newcommand{\pbare}{\bar{p}\Rightarrow e}
\newcommand{\eebar}{\overline{E\Rightarrow e}}
\newcommand{\eepbar}{\overline{E'\abar\Rightarrow e'}}
\newcommand{\eabar}{\overline{E\abar\Rightarrow e'}}
\newcommand{\exbar}{\overline{E\xbar\Rightarrow e}}
\newcommand{\exbarp}{\overline{E\xbar\Rightarrow e'}}
\newcommand{\abar}{\bar{a}}
\newcommand{\expbar}{\bar{e}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\vbar}{\bar{\nu}}
\newcommand{\ebar}{\overline{E}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\alabel}[1]{\quad\text{#1}}
\newcommand{\sep}{\;\mid\;}
\newcommand{\record}[2]{
  \{\:\beta#1: #2\; ;\;\ldots\;;\; \beta#1: #2\:\}_{\overline{\alpha}}}
\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\canbeta}[1]{\betabar\:\lozenge\:#1}
\newcommand{\fun}[3]{\lambda x:#1\:#2.\: #3}
\newcommand{\funreg}{\fun{\reg}{\tau}{e}}
\newcommand{\funghost}{\fun{\ghost}{\tau}{e}}

%%% semantics %%%
\newcommand{\state}{\delta\cdot\mu}
\newcommand{\statep}{\mu'}
\newcommand{\statepp}{\mu''}
\newcommand{\stated}[1]{\delta[#1]\cdot\mu}
\newcommand{\murule}[1]{\state\cdot #1}
\newcommand{\muprule}[1]{\statep\cdot #1}
\newcommand{\mupprule}[1]{\statepp\cdot #1}
\newcommand{\trans}[2]{#1\Downarrow #2}
\newcommand{\transco}[2]{#1\Downarrow^{\textsf{co}} #2}
\newcommand{\cxt}[2]{\trans{\murule{#1}}{\muprule{#2}}}
\newcommand{\cxtp}[2]{\trans{\murule{#1}}{\mupprule{#2}}}
\newcommand{\cxtco}[2]{\transco{\murule{#1}}{\muprule{#2}}}
\newcommand{\cxtcop}[2]{\transco{\murule{#1}}{\mupprule{#2}}}
\newcommand{\cxtcod}[1]{\transco{\murule{#1}}{\diverges}}
\newcommand{\cxtcodp}[1]{\transco{\muprule{#1}}{\diverges}}
\newcommand{\abort}{\texttt{abort}}

%%% progress %%%
\newcommand{\progdeltamu}[1]{#1\downarrow}
\newcommand{\prog}[1]{\progdeltamu{#1}}
\newcommand{\progrule}[2]{\inferrule*[Right=(#1)]{ }{\prog{#2}}}

%%% typing %%%
\newcommand{\dgste}[5]{#1\cdot #2\cdot #3\vdash #4 : #5}
\newcommand{\dgte}[4]{\dgste{#1}{#2}{\Sigma}{#3}{#4}}
\newcommand{\gte}[3]{\dgste{\Delta}{#1}{\Sigma}{#2}{#3}}
\newcommand{\nogte}[2]{\dgste{\Delta}{\emptyset}{\Sigma}{#1}{#2}}
\newcommand{\nogste}[3]{\dgste{\Delta}{\emptyset}{#1}{#2}{#3}}
\newcommand{\gste}[4]{\dgste{\Delta}{#1}{#2}{#3}{#4}}
\newcommand{\dte}[3]{\dgste{#1}{\Gamma}{\Sigma}{#2}{#3}}
\newcommand{\te}[2]{\dgte{\Delta}{\Gamma}{#1}{#2}}
\newcommand{\tp}[2]{\vdash #1 : #2}
\newcommand{\ori}[2]{\underset{#1}{\bigsqcup}#2}
\newcommand{\disji}[2]{\underset{#1}{\bigcup}#2}
\renewcommand{\sup}[2]{#1\sqcup#2}
\newcommand{\reg}{\texttt{reg}}
\newcommand{\ghost}{\texttt{ghost}}
\newcommand{\absurd}{\mathtt{absurd}}
\newcommand{\raises}{{\tt raises}}
\newcommand{\unit}{{\tt Unit}}
\newcommand{\bool}{{\tt Bool}}
\newcommand{\diverges}{{\tt div}}
\newcommand{\try}{{\tt try}}
\newcommand{\with}{{\tt with}}
\newcommand{\qqquad}{\qquad\qquad\quad}
\newcommand{\poly}{\langle\alphabar\rangle}
% \newcommand{\inst}{\langle\taubar\rangle}

%%% extraction %%%
\newcommand{\extarg}[2]{\mathcal{E}_{#1}(#2)}
\newcommand{\extbeta}[1]{\extarg{\betabar}{#1}}
\newcommand{\extkappa}[1]{\extarg{\kappa}{#1}}
\newcommand{\extsigma}[1]{\extarg{\sigma}{#1}}
\newcommand{\extkappap}[1]{\extarg{\kappa'}{#1}}
\newcommand{\ext}[1]{\extarg{}{#1}}
\newcommand{\extghost}[1]{\extarg{\ghost}{#1}}
\newcommand{\extreg}[1]{\extarg{\reg}{#1}}
\newcommand{\masksub}[2]{#1\sqsubseteq#2}
\newcommand{\notmasksub}[2]{#1\not\sqsubseteq#2}
\newcommand{\masklt}[2]{#1\sqsubset#2} \newcommand{\exttry}[1]{
  \overline{E\xbar_{\restriction{#1}}\Rightarrow\extbeta{e'}}}
\newcommand{\extp}{\overline{\ext{\pbar}\Rightarrow\extsigma{e}}}
\newcommand{\extrec}[2]{\ext{ \{\:\beta_1#1_1: #2_1\; ;\;\ldots\;;\;
    \beta_n#1_n: #2_n\:\}}} \newcommand{\extrecreg}[2]{ \{\:\overline{{\tt
      reg}\:#1_i : #2_i}\:\}_{\alphabar}} \newcommand{\mask}[1]{\mathcal{M}(#1)}
\newcommand{\exttyp}[1]{
  \dgste{\mathcal{E}(\Delta)}{\mathcal{E}(\Gamma)}{\Sigma}
  {\mathcal{E}_{\betabar}(e)}{\mathcal{E}_{\betabar}(#1)}}
\renewcommand{\restriction}[1]{\mathord{\upharpoonright}#1}
\newcommand{\extenv}{\ext{\Delta\cdot\Gamma\cdot\Sigma}}
\newcommand{\extte}[2]{\extenv\vdash #1 : #2}
\newcommand{\extdgste}[5]{\ext{#1}\cdot\ext{#2}\cdot\ext{#3}\vdash #4 : #5}
\newcommand{\cxtext}[2]{\ext{\delta}\cdot\ext{\mu}\cdot #1\Downarrow #2}
\newcommand{\cxtpext}[2]{\ext{\delta}\cdot\ext{\mu'}\cdot #1\Downarrow #2}
\newcommand{\cxtppext}[2]{\ext{\delta}\cdot\ext{\mu''}\cdot #1\Downarrow #2}
\newcommand{\cxtcodext}[1]{\ext{\delta}\cdot\ext{\mu}\cdot
  #1\Downarrow^{\textsf{co}}\diverges}
\newcommand{\cxtcodextp}[1]{\ext{\delta}\cdot\ext{\mu'}\cdot
  #1\Downarrow^{\textsf{co}}\diverges}

%%% defs & theorems %%%
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{prop}[theorem]{Property}
% \newtheorem{corollary}{Corollary}[theorem]
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]

% \newcommand{\case}[1]{\paragraph{case \color{blue}{(\textsc{#1}).}}}
% \newcommand{\rulename}[1]{{\color{blue}{\textsc{(\textbf{#1})}}}}

